On Computing the Shapley Value in Bankruptcy Games -llustrated by Rectified Linear Function Game-

In this research, we discuss a problem of calculating the Shapley value in bankruptcy games. We show that the decision problem of computing the Shapley value in bankruptcy games is NP-complete. We also investigate the relationship between the Shapley value of bankruptcy games and the Shapley-Shubik index in weighted voting games. The relation naturally implies a dynamic programming technique for calculating the Shapley value. We also present two recursive algorithms for computing the Shapley value: the first is the recursive completion method originally proposed by O'Neill, and the second is our novel contribution based on the dual game formulation. These recursive approaches offer conceptual clarity and computational efficiency, especially when combined with memoisation technique. Finally, we propose a Fully Polynomial-Time Randomized Approximation Scheme (FPRAS) based on Monte Carlo sampling, providing an efficient approximation method for large-scale instances.

==> Proofs/PropVecCore.tex <==
\begin{proof}
As $\Hprop{\Vec{y}}$ is an imputation, we only need to show that it satisfies coalitional rationality 
 $[\sum_{i \in S}y_i \geq v(S) \; (\forall S \subseteq N)]$.

\begin{enumerate}
    \item If $\sum_{i \in S} w_i < w_0$,
 then the non-negativity of $\Hprop{\Vec{y}}$ implies $\sum_{i \in S} \Hprop{y_i} \geq 0=v(S)$.
    \item In the remained case that $\sum_{i \in S} w_i \geq w_0$,
    we have the following inequalities
\[
    \sum_{i \in S} \Hprop{y_i} - v(S) 
    = \frac{W-w_0}{W}\sum_{i \in S} w_i 
       - \left( -w_0+\sum\limits_{i \in S}w_i \right) 
    =w_0 \left( 1-\frac{\sum_{i \in S}w_i}{W} \right) \geq 0.
\]
\end{enumerate}
%Therefore
%$\sum\limits_{i \in S}y_i \geq v(S) \;\;
%  (\forall S \subseteq N)$
%holds.
\end{proof}

==> Proofs/PropVecImp.tex <==
\begin{proof}
1. Each player $i \in N$ satisfies that $\Hprop{y_i} \geq 0$ and 
$ \Hprop{y_i} - (-w_0 + w_i) 
    = w_0 \left(1 - \frac{w_i}{W}\right) 
    \geq 0$. 
The above inequalities directly imply that 
 $ \Hprop{y_i} \geq \max \{0, -w_0+w_i \}=v(\{i\}).$

2. The definition of $\Hprop{\Vec{y}}$ directly implies that 
\[
\sum_{i \in N} \Hprop{y_i}
 = \frac{(W - w_0)}{W} \sum_{i \in N}w_i = W - w_0 = v(N).
\]
\end{proof}

==> Proofs/bankruptcy.tex <==
\begin{proof}
Let $(N, v)$ be a rectified linear function game with:
\begin{center}
$v(S) = \max \left\{ 0, -w_0 + \sum\limits_{i \in S} w_i \right\} $
\end{center}

Define a bankruptcy game $(N, E, d)$ where:
\begin{itemize}
\item $E = W - w_0 = \sum_{i \in N} w_i - w_0$
\item $d_i = w_i$ for all $i \in N$
\end{itemize}

For any coalition $S \subseteq N$, the value in the bankruptcy game is:
\begin{align*}
v_E^d(S) &= \max \left\{ 0, E - \sum\limits_{i \in N \setminus S} d_i \right\} 
 = \max \left\{ 0, (W - w_0) - \sum\limits_{i \in N \setminus S} w_i \right\} \\
&= \max \left\{ 0, W - w_0 - \left( W - \sum\limits_{i \in S} w_i \right) \right\} 
 = \max \left\{ 0, -w_0 + \sum\limits_{i \in S} w_i \right\} 
 = v(S)
\end{align*}

Conversely, given a bankruptcy game $(N, v_E^d)$, we can define a rectified linear function game with $w_i = d_i$ for all $i \in N$ and $w_0 = \sum\limits_{i \in N} d_i - E$. 
\end{proof}

==> Proofs/merg.tex <==
\begin{Lemma}\label{lemma:merg}
Consider a bankruptcy game defined by $[E; w_1, \ldots, w_n]$, 
and let $\Merg(\pi,i)$ denote the marginal contribution of player $i \in N$ 
for a permutation $\pi$ in this game.  

Similarly, consider a weighted voting game defined by $[q; w_1, \ldots, w_n]$, 
and let $\Mergq(\pi,i)$ denote the marginal contribution of player $i \in N$ 
for a permutation $\pi$ in this game.

Then, the following holds:
\[
\Merg(\pi,i) = \sum_{q = w_0+1}^{W}\Mergq(\pi,i),
\]
where $W = w_1 + \cdots + w_n$.
\end{Lemma}



\begin{proof}
It is obvious that $\Merg(\pi,i) = \sum_{q = w_0+1}^{W}\Mergq(\pi,i)=0$ holds when $w_i=0$.  
We now turn to the case $w_i > 0$. 

Let $s = \sum_{j \in \text{Prc}(\pi,i)} w_j$.  
We divide the proof into three cases depending on the value of $w_0$.



\item Case 1: $0 \le w_0 \le s$. \\
First, by the definition of $\Mergq$, we have
\[
\sum_{q=w_0+1}^W\Mergq(\pi,i)=\sum_{q=s+1}^{s+w_i}1 = w_i.
\]
In addition, we obtain
\begin{align*}
\Merg(\pi,i)& =\max(0,-w_0+s+w_i) - \max(0,-w_0+s) 
\\ &= (-w_0+w_i+s) - (-w_0+s) 
\\ &= w_i.
\end{align*}

\item Case 2: $s < w_0 < s+w_i$. \\
By the definition of $\Mergq$, we have
\[
\sum_{q=w_0+1}^W\Mergq(\pi,i)=\sum_{q=w_0+1}^{s+w_i}1 = -w_0+w_i+s.
\]
Also, 
\begin{align*}
\Merg(\pi,i)&=\max(0,-w_0+s+w_i) - \max(0,-w_0+s) 
\\&= (-w_0+w_i+s) - 0 
\\&= -w_0+w_i+s.
\end{align*}

\item Case 3: $s+w_i \le w_0 \le W$. \\
In this case, player $i$ cannot be a pivot player for any quota $q \in [w_0+1,W]$.  
Therefore,
\[
\sum_{q=w_0+1}^W\Mergq(\pi,i)=0.
\]
Moreover,
\[
\Merg(\pi,i)=\max(0,-w_0+s+w_i) - \max(0,-w_0+s) 
= 0 - 0 
= 0.
\]

This completes the proof.
\end{proof}


==> Proofs/ssindex.tex <==
\begin{Theorem}\label{Theorem:ssindex}
Consider a bankruptcy game defined by 
    $\BG[E; \Vec{w}]$  
    defined by integer vector $\Vec{w}$  
    and a positive integer estate $E$.
Then the Shapley value of player $i \in N$, denoted by $\phi_i$, satisfies
\[
\phi_i = \sum_{q = w_0+1}^{W} \phi_i^{\langle q \rangle},
\]
where $W = w_1 + \cdots + w_n$.  
Here, $\phi_i^{\langle q \rangle}$ denotes the Shapley–Shubik index of player $i$ 
in the weighted voting game defined by $[q;w_1, w_2, \ldots, w_n]$.
\end{Theorem}



\begin{proof}
From Lemma~\ref{lemma:merg},
\begin{align*}
\phi_i
= \sum_{\pi \in \Pi_N} \Merg(\pi,i) = \sum_{\pi \in \Pi_N} \sum_{q=w_0+1}^W \Mergq(\pi,i) &= \sum_{q=w_0+1}^W \sum_{\pi \in \Pi_N} \Mergq(\pi,i) \\
&= \sum_{q=w_0+1}^W \phi_i^{<q>}.
\end{align*}
\end{proof}


ーーーーーーーーーーーーーーーーーーーーーー
{\color{yellow} 
ーーーーーーーーー old version ーーーーーーーーーーーーーー

\begin{Theorem}\label{Theorem:ssindex2}
Let $\Vec{w}$ be a vector of positive integers, 
    and $E$ be a positive integer satisfying
    $E + 1 < W := \sum_i w_i$. 
Define $\phi^+$ and $\phi$ as the Shapley values corresponding to the bankruptcy games 
$\BG[E+1; \Vec{w}]$ and $\BG[E; \Vec{w}]$, respectively.
The difference between the Shapley values defined above 
    satisfies the identity
\begin{equation} \label{ParametricAnalysis}
    \phi^+ - \phi =\varphi^{\langle W-E \rangle},
\end{equation}
where $\varphi^{\langle W-E \rangle}$ is 
    the Shapley-Shubik index 
    defined by $WVG[W-E;\Vec{w}].$
\end{Theorem}

\begin{proof}
Let $(N,v^+)$, $(N,v)$ and $(N,v^{\langle W-E \rangle})$ 
be characteristic function form games 
    defined by 
    $\BG [E+1;\Vec{w}]$, $\BG [E; \Vec{w}]$ and 
     $\WVG [W-E;\Vec{w}]$, 
    respectively. 
 First, we show the equalities 
    $v^+(S)- v(S)=v^{\langle W-E \rangle} (S)$ 
    $(\forall S \subseteq N).$



If coalition $S$ satisfies 
    $\sum_{i\in S} w_i \leq W-E-1$, 
    then $v^+ (S)=0$, $v(S)=0$ and
    $v^{\langle W-E \rangle} (S)=0$, 
    which implies 
    $v^+(S)- v(S)=0=v^{\langle W-E \rangle} (S).$ 
Consider the case that $\sum_{i\in S} w_i \geq W-E$.
Then, we have that
\[
    v^+(S)-v(S)=
    \left( 
        \left (\sum_{i\in S} w_i \right) - (W-E-1)
    \right)
    -\left( 
        \left( \sum_{i\in S} w_i \right) - (W-E)
    \right) =1=v^{\langle W-E \rangle }(S).
\]

Thus, we have that
    $ v^+=v+v^{\langle W-E \rangle}$
    and the additivity (law of aggregation~\cite{shapley1953value})
of the Shapley value implies the desired result.
\end{proof}

\begin{Cor}
%    Consider a bankruptcy game $(N,v)$ defined by 
%   $\BG[E; \Vec{w}],$  
%    where $\Vec{w}$ is a vector of positive integers 
%    and $E$ is a positive integer satisfying $0<E<W$. 
The Shapley value $\phi$ of $\BG[E; \Vec{w}]$  
    satisfies
$
 \phi= \sum_{q = W-E+1}^{W} \varphi^{\langle q \rangle}.
$
\end{Cor}
% \input{Proofs/ssindex}

\begin{proof}
Let $\phi^{\bullet}$ be the Shapley value of 
     $\BG [1; \Vec{w}].$
Then, by telescoping the sum 
    in equality~(\ref{ParametricAnalysis}), 
    we obtain that 
\begin{eqnarray*}
 \phi &=& \sum_{q=W-E+1}^{W-1} \varphi^{\langle q \rangle}
    +\phi^{\bullet}
    =\sum_{q=W-E+1}^{W-1} \varphi^{\langle q \rangle}
    +\left( \frac{1}{n} \right) (1,1,\ldots ,1) \\
    &=& \sum_{q=W-E+1}^{W-1} \varphi^{\langle q \rangle}
    +\varphi^{\langle W \rangle}
    =\sum_{q=W-E+1}^{W} \varphi^{\langle q \rangle}.
\end{eqnarray*}
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From the above Corollary, 
    one can compute the Shapley value of a bankruptcy game 
    by executing an algorithm for computing 
    the Shapley–Shubik index of a weighted voting game 
    $E (=W-w_0)$ times.
Furthermore, %as in Aziz~\cite{aziz2013computation}, 
    by modifying the algorithm for computing 
    the Shapley–Shubik index, 
    it may be possible to construct a more efficient method than simply running it $E$ times.

In the following, we describe an algorithm
    based on the dynamic programming technique,
    whose time complexity is bounded by $O(n^2 W)$ for each player. 
The definition of weighted voting game $(N,v_q)$ implies that
\[
    \begin{array}{rcl}
    \phi_i^{\langle q \rangle}&=&\displaystyle 
    \sum_{S\subseteq N \setminus \{i\}}
    \frac{|S|! (n-|S|-1)!}{n!}(v_q(S \cup \{i\})-v_q(S)) \\
    &=& \displaystyle 
    \sum_{t=1}^{n-1} \sum_{w=q-w_i}^{q-1}
    \frac{t! (n-t-1)!}{n!} c_i (w,t),
    \end{array} 
\]
where 
\[
    c_i (w,t)
    =\left\{ \begin{array}{ll} 
    \displaystyle 
    \# \left\{S \subseteq N\setminus \{i\} 
        \left|  \sum_{i \in S} w_i =w \mbox{ and } |S|=t 
        \right. \right\} 
        & (\mbox{ if } 1\leq w\leq W \mbox{ and } 1\leq t \leq n), \\
    0 & (\mbox{otherwise}).
    \end{array} \right.
\]

Theorem~\ref{Theorem:ssindex} implies that
\[
\begin{array}{rcl}
\phi_i %= \sum_{q = w_0+1}^{W} \phi_i^{\langle q \rangle}
&=& \displaystyle 
 \sum_{q = w_0+1}^{W} \sum_{t=1}^{n-1}  \sum_{w=q-w_i}^{q-1}
    \frac{t! (n-t-1)!}{n!} c_i (w,t) \\
&=& \displaystyle 
 \sum_{t=1}^{n-1} 
 \left( 
  \frac{t! (n-t-1)!}{n!}  
    \sum_{w = w_0+1-w_i}^{W-1} 
    \left(
        (\min\{ W, w+w_i\}- \max \{w+1, w_0+1\}) 
        c_i (w,t)
    \right)
 \right),  
 \end{array}
\]  
which allows us to compute the Shapley value $\phi_i$ 
in $O(nW)$ time using
the $W \times n$ matrix $C_i=(c_i(w,t)).$
An ordinary dynamic programming technique gives 
    an algorithm for calculating the matrix $C_i=(c_i(w,t))$
    in $O(n^2 W)$ time (see~\cite{matsui2000survey} for example).
Thus, there exists an algorithm for calculating 
    the Shapley value of a bankruptcy game 
    whose time complexity is bounded by $O(n^2 W)$ for each player. 

}

==> Proofs/superadditive.tex <==
\begin{proof}
We prove that $[\forall S, \forall T \subseteq N, 
 S \cap T = \emptyset \rightarrow  v(S)+v(T) \leq v(S \cup T)]$ holds.

\begin{enumerate}
\item  When $-w_0 + \sum\limits_{i \in S \cup T}w_i \leq 0$,
it is clear that $v(S)=v(T)=v(S\cup T) = 0$ holds. Therefore, $v(S)+v(T) \leq v(S \cup T)$
is satisfied.

\item Consider the case where $-w_0 + \sum\limits_{i \in S \cup T}w_i > 0$ is satisfied. 
The assumption $S \cap T=\emptyset$ directly implies the equality $\sum\limits_{i \in S \cup T}w_i = \sum\limits_{i \in S}w_i + \sum\limits_{i \in T}w_i$. 
Therefore, we have that 
\begin{align*}
v(S \cup T) &= -w_0 + \sum\limits_{i \in S \cup T}w_i 
=-w_0 + (\sum\limits_{i \in S}w_i + \sum\limits_{i \in T}w_i) \\
& \geq (-w_0+\sum\limits_{i \in S}w_i) + (-w_0+\sum\limits_{i \in T}w_i) 
=v(S)+v(T).
\end{align*}
\end{enumerate}
\end{proof}

==> Proofs/supermodular.tex <==
\begin{proof}
We prove that $[\forall S, \forall T \subseteq N, v(S)+v(T) \leq v(S \cup T) + v(S \cap T)]$ holds.

\begin{enumerate}
\item  When $v(S)=v(T) = 0$,
 the non-negativity of $v(S\cup T)$ and $v(S \cap T)$  leads to the desired inequality.

\item 
When $v(S)>0= v(T)$, 
we have that 
\[
v(S)+v(T)=-w_0 + \sum_{i \in S}w_i +0 
 \leq -w_0 + \sum_{i \in S \cup T}w_i 
 =v(S \cup T)=v(S \cup T) +v(S \cap T).
\]

\item We can similarly address the case that $v(T)>  0=v(S)$ with (2).

\item 
If $v(S)>0$ and $v(T)>0$ hold, 
    it directly implies $v(S \cup T) > 0$ and thus we have that  
\[
\begin{array}{ll}
 v(S \cup T)+ v(S \cap T)  - v(S) - v(T) \\
= \left( -w_0 + \sum\limits_{i \in S \cup T}w_i \right) + v(S \cap T)  
  - \left( -w_0 + \sum\limits_{i \in S}w_i \right) 
  - \left( -w_0 + \sum\limits_{i \in T}w_i \right) \\
 = v(S \cap T) -\left( - w_0 + \sum\limits_{i \in S \cap T}w_i \right) 
 \geq 0.
\end{array}
\]

\end{enumerate}
From the above, $v$ satisfies supermodularity.
\end{proof}

==> omitted.tex <==
\section{Equivalence to Bankruptcy Games}
In this section, we establish that rectified linear function games are equivalent to bankruptcy games, a well-studied class of cooperative games introduced by O'Neill (1982)\cite{o1982problem}.

A bankruptcy game involves a set of claimants $N = \{1, 2, \ldots, n\}$, their claims $d = (d_1, d_2, \ldots, d_n)$ where $d_i \geq 0$ for all $i \in N$, and an estate $E \geq 0$ to be divided among them. The bankruptcy game is represented by the tuple $(N, E, d)$, where the total claim exceeds the estate, i.e., $\sum_{i \in N} d_i > E$.

The corresponding bankruptcy game $(N, v_E^d)$ is defined as:
\begin{center}
$v_E^d(S) = \max \left\{ 0, E - \sum\limits_{i \in N \setminus S} d_i \right\}$ for all $S \subseteq N$.
\end{center}

We now prove that rectified linear function games and bankruptcy games represent the same class of cooperative games.

\begin{Theorem}\label{Theorem:bankruptcy}
For any rectified linear function game $(N, v)$ defined by 
a vector $(w_0; w_1, \ldots , w_n)$, 
there exists a bankruptcy game $(N, v_E^d)$ that is equivalent to $(N, v)$, and vice versa.
\end{Theorem}

\input{Proofs/bankruptcy}

\section{Basic Properties}\label{Section:Basic}

First, we demonstrate the superadditivity and supermodularity of the characteristic function of rectified linear function games.

\begin{Lemma}\label{Theorem:superadditive}
The rectified linear function game $(N, v)$ satisfies superadditivity, i.e., 
\linebreak  $[\forall S, \forall T \subseteq N, 
 S \cap T = \emptyset \rightarrow  v(S)+v(T) \leq v(S \cup T)]$ holds.
\end{Lemma}

% \input{Proofs/superadditive}

\begin{Lemma}\label{Theorem:supermodular}
The rectified linear function game $(N, v)$ satisfies supermodularity, 
i.e.,  $[\forall S, \forall T \subseteq N, v(S)+v(T) \leq v(S \cup T) + v(S \cap T)]$ holds.
\end{Lemma}

%\input{Proofs/supermodular}

%\section{Imputations in Rectified Linear Function Games}\label{section5}

Next, we discuss imputations in rectified linear function games.
One of the key challenges in characteristic function form games is how to allocate the total benefit generated by cooperation among players.
In this paper,
we denote the payoff vector in rectified linear function games as
$\boldsymbol{y}=(y_1,y_2,\ldots ,y_n)$.

In the following, 
we discuss the payoff vector 
    $\Hprop{\Vec{y}}=(\Hprop{y_1}, \Hprop{y_2}, \ldots ,\Hprop{y_n})$
    called  a {\em proportional distribution},  
    defined by 
\begin{align}
\Hprop{y_i} =\frac{v(N)}{W}w_i=
  \frac{(W - w_0)}{W}w_i
  \;\;\; (\forall i \in N).\label{def:PropImp}
\end{align}

\smallskip

\begin{Lemma}\label{Theorem:PropVecImp}
 The payoff vector $\Hprop{\Vec{y}}$ satisfies the followings; 
\begin{enumerate}
\item $\Hprop{y_i} \geq v(\{i\}) \;\;\; (\forall i \in N)$,  
\item $\sum_{i \in N} \Hprop{y_i} = v(N)$.
\end{enumerate}
\end{Lemma}

%\input{Proofs/PropVecImp}

From the above, $\Hprop{\Vec{y}}$ is an {\em imputation}.
%In the following, we call  $\Hprop{\Vec{y}}$ as a {\em proportional distribution}.  

\smallskip 

\begin{Theorem}\label{Theorem:PropVecCore}
The proportional distribution $\Hprop{\Vec{y}}$ belongs to the core.
Thus, the core is non-empty.
\end{Theorem}

%\input{Proofs/PropVecCore}
